KnowAgent: Knowledge-Augmented Planning for LLM-Based Agents

Large Language Models (LLMs) have demonstrated great potential in complex reasoning tasks, yet they fall short when tackling more sophisticated challenges, especially when interacting with environments through generating executable actions. This inadequacy primarily stems from the lack of built-in action knowledge in language agents, which fails to effectively guide the planning trajectories during task solving and results in planning hallucination. To address this issue, we introduce KnowAgent, a novel approach designed to enhance the planning capabilities of LLMs by incorporating explicit action knowledge. Specifically, KnowAgent employs an action knowledge base and a knowledgeable self-learning strategy to constrain the action path during planning, enabling more reasonable trajectory synthesis, and thereby enhancing the planning performance of language agents. Experimental results on HotpotQA and ALFWorld based on various backbone models demonstrate that KnowAgent can achieve comparable or superior performance to existing baselines. Further analysis indicates the effectiveness of KnowAgent in terms of planning hallucinations mitigation. Code is available in https://github.com/zjunlp/KnowAgent.

==> tabs/algorithm.tex <==
% % \begin{algorithm}
% %   \caption{Trajectory Generation and Self-Learning for Task Resolution}
% %   \KwIn{\(AK\): Action Knowledge as a collection of Actions \( A \) and Action Rules \( R \); \( D_0 \): Initial training set}
% %   % \KwOut{Updated Models \( M_1, M_2, \ldots \); Generated Trajectories \(T = {\tau_1}\)}
  
% %   \textbf{Main Loop:} \\
% %   \For{\( iteration = 1 \) \KwTo \( n \)}{
% %     Perform experiments in initial training set \( D_0 \), obtaining a simulated trajectory \\
% %     Train model with new trajectory to get \( M_{iteration} \) \\
% %     Evaluate \( M_{iteration} \) in \( D_0 \) to generate a new trajectory \\
% %     Merge new trajectory with previous one \\
% %     Fine-tune \( M_{iteration} \) with merged trajectory to obtain \( M_{iteration+1} \) \\
% %   }
  
% %   \KwRet{Updated Models \( M \), Generated Trajectories}
% %   \label{algo:self_learning_trajectory}
% % \end{algorithm}


% \begin{algorithm}
%   \caption{Knowledgeable Self-Learning Process}
%   \KwIn{\(AK\): Action Knowledge, comprising a set of Actions \( A \) and Action Rules \( R \); \( D_0 \): Initial Training Set;}
  
%   \textbf{Initialize:} The initialize model: \( M_0 \) \\
%   % The initial trajectories: \( T_{0} = M_0(AK,D_0) \) ;  \\
  
%   \For{\( i \gets 0 \) \KwTo \( N \)}{
%       \eIf{\( i = 0 \)}{
%            \Comment{Trajectory Generation}
%             \( T_i \leftarrow M_{i}(AK, D_0) \) \\
%              \Comment{Model Fine-tuning}
%             \( M_i \leftarrow Tune (T_i,M_{i}) \) \\
%       }
%        {
%         \Comment{Model Evaluation}
%         \( T_i \leftarrow Evaluate(D_0, M_i) \)
        
%         \Comment{Trajectory Merging and Filtering}
%         \( T_i \leftarrow MF( T_{i-1}, T_i)\)\\
        
%         \Comment{Model Fine-tuning}
%          \( M_{i+1} \leftarrow Tune (T_i,M_{i}) \) \\
%       }
%   }
  
%   \KwRet{Updated Models \( M \)}
%   \label{algo:self_learning_trajectory}
% \end{algorithm}

\begin{algorithm}[t]
\small
\caption{Trajectory Synthesis and Knowledgeable Self-Learning}
\label{algorithm1}
\KwIn{\(AK_m\): Task-specific Action Knowledge from \(Action\;KB\), including a set of actions \(E_a\) and action rules \(R\); \(D_0\): Initial training set; \(D_{\text{test}}\): Testing set.}

\KwOut{Optimized models \(M = \{M_1, M_2, \ldots\}\).}

\textbf{Initialize:} Model \(M_0\).

\For{\(i = 0\) \textbf{until} test performance stabilizes}{
    \If{\(i = 0\)}{
        \tcpo{Synthesize initial trajectories.}\par
        \(T_i \leftarrow Traj(M_i,AK_m, D_0)\)\par
        \vspace{2pt}
        \tcpo{Fiter trajectories.}\par
        \(T_i' \leftarrow Filter(T_i, AK_m)\)\par
        \vspace{2pt}
        \tcpo{Initial fine-tuning.}\par
        \(M_{i+1} \leftarrow Tune(T_i', M_i)\)
    }
    \Else{
        \tcpo{Synthesize trajectories.}\par
        \(T_i \leftarrow Traj(M_i,AK_m, D_0)\)\par
        \vspace{2pt}
        \tcpo{Filter and merge trajectories.}\par
        \(T_i' \leftarrow FilterAndMerge(T_i,T_{i-1}, AK_m)\)\par
        \vspace{2pt}
        \tcpo{Further fine-tuning.}\par
        \(M_{i+1} \leftarrow Tune(T_i', M_i)\)
    }
    \tcpo{Performance check}\par
    \If{\(\Delta Perf(M_{i+1}, M_i, D_{test}) \leq \epsilon\)}{
        \textbf{break}
    }
}
\Return{Optimized models \(M\)}
\label{algo:self_learning}
\end{algorithm}

==> tabs/experiment_ablation.tex <==
% \begin{wraptable}{r}{0.7\textwidth}
\begin{table}[!htbp]
\centering
\captionsetup{width=1\textwidth}
% \small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{r c cc}
\toprule
  \textbf{Models} & \textbf{Pre-trained} &  \multicolumn{1}{c}{\textbf{Iter 1}} & \multicolumn{1}{c}{\textbf{Iter 2}}\\
\midrule
\rowcolor{lightgray}
\multicolumn{4}{c}{\textit{Llama-2-7b}} \\
\midrule

{\ours} & 28.77 & 27.64  &33.47  \\
\textit{w/o KB} &27.79 &25.60 &31.41  \\
\midrule
\rowcolor{lightgray}
\multicolumn{4}{c}{\textit{Llama-2-13b}} \\
\midrule
{\ours}&29.00  &31.14  & 39.26 \\
\textit{w/o Act-KB}&28.68  &29.79  &35.10  \\
\midrule
\rowcolor{lightgray}
\multicolumn{4}{c}{\textit{Llama-2-70b}} \\
\midrule
{\ours}&41.08  &44.03    &48.14   \\
\textit{w/o KB}&40.44  &45.56  &45.80   \\
\bottomrule
\end{tabular}
\label{tab:ablation_llama2}
\caption{Ablation on Action Knowledge Base}
\end{table}
% \end{wraptable}

==> tabs/experiment_basemodel.tex <==
\begin{table}[!htbp]
\centering
\captionsetup{width=0.32\textwidth}
% \small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l c cccc}
\toprule
  \textbf{KnowAgent} & \textbf{Pre-trained} &  \multicolumn{1}{c}{\textbf{Iter 1}} & \multicolumn{1}{c}{\textbf{Iter 2}} & \multicolumn{1}{c}{\textbf{Iter 3}}& \multicolumn{1}{c}{\textbf{Iter 4}}\\
\midrule
\textit{vicuna-7b} &24.01  &24.17  &28.31 &30.12 &32.28 \\
 \textit{mistral-7b}&21.25   &25.66    &30.65 &30.73 &33.42 \\
 \textit{llama-7b}&28.77  &27.64    &33.47  &32.65 &33.50 \\
\bottomrule
\end{tabular}
\caption{Ablation on Base Model}
\label{tab:ablation_base_model}
\end{table}

==> tabs/experiment_gpt.tex <==
% % \begin{wraptable}{r}{0.7\textwidth}
% \begin{table}[!htbp]
% \centering
% \captionsetup{width=0.48\textwidth}
% % \small
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{r| c cc|c}
% \toprule
%   \textbf{Models} & Easy &  Medium& Hard& \multicolumn{1}{c}{\textbf{Average}}\\
% \midrule
% \rowcolor{lightgray}
% \multicolumn{5}{c}{\textit{gpt-3.5-turbo}} \\
% \midrule
%  \ours &47.68  &42.97   &34.51    &41.72   \\
%  \textit{w/o KB} &49.71   &40.25   &32.80  &40.92   \\
% \midrule
% \rowcolor{lightgray}
% \multicolumn{5}{c}{\textit{gpt-4-0616}} \\
% \midrule
%  \ours &65.89  &65.03    &55.32 &62.08   \\
%  \textit{w/o KB} &63.96  &64.44  &56.15 &61.52   \\
% \bottomrule
% \end{tabular}
% \caption{Ablation on GPT3.5 and GPT4}
% \label{tab:ablation_gpt}
% \end{table}
% % \end{wraptable}

\begin{table}[!htbp]
\centering
\captionsetup{width=0.45\textwidth}
% \small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{r| c c}
\toprule
  \textbf{Models} &\textit{gpt-3.5-turbo} & \textit{gpt-4-0616}\\
\midrule
 \ours     &41.72  &62.08  \\
 \textit{- Action KB}   &40.92  &61.52   \\
\bottomrule
\end{tabular}
\caption{Ablation study on Action Knowledge within GPT-3.5 and GPT-4.}
\label{tab:ablation_gpt}
\end{table}

==> tabs/experiment_iter.tex <==
% \begin{wraptable}{r}{0.65\textwidth}
\begin{table*}
    \centering
    \scalebox{1}{
   \begin{tabular}{l|c|ccc|c} \toprule 
    % \multirow{2}{*}{\textbf{Model}} 
    % & \multicolumn{4}{c}{\textbf{HotpotQA}} \\ \cmidrule(lr){2-5}
    % &  Easy & Medium & Hard & Average \\ \midrule
    \multirow{1}{*}{\textbf{Model}} 
    &\multirow{1}{*}{\textbf{Method}} 
    &  Easy & Medium & Hard & \textbf{Average} \\ \midrule
    % \rowcolor[gray]{0.95} \multicolumn{6}{c}{\textbf{Prompting} } \\ \midrule
    \multirow{4}{*}{\texttt{KnowAgent-\textcolor{light_blue}{7B}}}
    & Iter-1
     &37.7 & 25.00& 20.21 &27.64  \\
    & Iter-2
     & 40.80&32.48 & 27.12 & 33.47 \\
    & Iter-3
     & 44.93&23.17 &29.86  &32.65  \\
    & Iter-4
     &45.78 &30.47 &24.25  & 33.50 \\\midrule
    
    % \rowcolor[gray]{0.95} \multicolumn{6}{c}{\textbf{Fine-tuning}}  \\ \midrule
    \multirow{4}{*}{\texttt{KnowAgent-\textcolor{medium_blue}{13B}}}
    & Iter-1
     &40.86 &29.33 &23.21  &31.14  \\
    & Iter-2
     &46.96 &37.60 &33.20  &39.26  \\
    & Iter-3
     & 46.13&32.92 &31.83  &36.96  \\
    & Iter-4
     &49.72 &32.37 &33.94  &39.67  \\
    \bottomrule
    \end{tabular}}
    \caption{Iteration Analysis}
    \label{tab:iteration}
\end{table*}
% \end{wraptable}

==> tabs/main_result1.tex <==
\begin{table*}[t!]
\centering
\renewcommand\arraystretch{1.0}
\scalebox{0.9}{
\begin{tabular}{cllccccc}
\hline
\toprule
{\multirow{2}{*}{\textbf{Backbone}}}
& {\multirow{2}{*}{\textbf{Strategy}}} 
& {\multirow{2}{*}{\textbf{Method}}} 
& \multicolumn{4}{c}{\textbf{HotpotQA}} 
& {\multirow{2}{*}{\textbf{ALFWorld}}}  \\
\cmidrule(lr){4-7} 
 & & &\textit{Easy} & \textit{Medium} & \textit{Hard} & \textit{Average} &\\
\Xhline{1px}
\multirow{6}{*}{\makecell{Llama-2\\7B-chat}}
     & Prompting
    & CoT~\cite{cot}
     & 35.80 & 26.69 & 18.20 & 26.90 &- \\
     & Prompting
    & ReAcT~\cite{react}
     & 25.14 & 19.87 & 17.39 & 20.80 & 1.49\\
     & Prompting
    & Reflexion~\cite{reflexion}
     & 35.55 & 28.73 & 24.35 & 29.54& 5.97 \\
     & Fine-tuning 
    & FiReAct~\cite{fireact}
     & 40.56 & 31.70 & 24.13 & 32.13 & 25.38 \\
     \cmidrule(lr){2-8}
     & Fine-tuning 
     % & Fine-tune
    & \textbf{\ours}-\textcolor{light_blue}{7B}
     &\textbf{40.80} &\textbf{32.49} &\textbf{27.12} &\textbf{33.47}  &\textbf{29.35}\\
    %  & Fine-tuning 
    % &  {\ours}-\textcolor{light_blue}{7B} (distilled)
    %  &34.30  &20.63  &20.72  &25.22 &18.66 \\
\Xhline{1px}
\multirow{6}{*}{\makecell{Llama-2\\13B-chat}}
    & Prompting
    & CoT~\cite{cot}
    & 37.90 & 25.28 & 21.64 & 28.27 & -   \\
    & Prompting
    & ReAcT~\cite{react}
    & 28.68 & 22.15 & 21.69 & 24.17 &20.90\\
    & Prompting
    & Reflexion~\cite{reflexion}
    & 44.43 & 37.50 & 28.17 & 36.70 & 34.33\\
     & Fine-tuning 
    % & Fine-tune 
    & FiReAct~\cite{fireact}
    & \textbf{51.95} & 33.93 & 28.88 & 38.26 & 50.37 \\
    \cmidrule(lr){2-8}
     & Fine-tuning 
    % & Fine-tune 
    & \textbf{\ours}-\textcolor{medium_blue}{13B} 
    &46.97 &\textbf{37.60} &\textbf{33.22} &\textbf{39.26}  &\textbf{58.71} \\
    % &\textbf{52.24}\\
     % & Fine-tuning 
    % & Fine-tune 
    % & {\ours}-\textcolor{medium_blue}{13B} (distilled)
    %  &28.62      &24.70   &23.85   &25.72 &51.49  \\
\Xhline{1.2px}
\multirow{6}{*}{\makecell{Llama-2\\70B-chat}}
    & Prompting
    & CoT ~\cite{cot}
    & 45.37 & 36.33 & 32.27 & 37.99 &- \\
    & Prompting
    & ReAcT~\cite{react}
    & 39.70 & 37.19 & 33.62 & 36.83 &55.22\\
    & Prompting
    & Reflexion~\cite{reflexion}
    & 48.01 & 46.35 & 35.64 & 43.33 &69.40\\
     & Fine-tuning 
    % & Fine-tune
    & FiReAct~\cite{fireact}
    & 51.96 & 47.56 & \textbf{44.60} & 48.04 & 77.61 \\ 
    \cmidrule(lr){2-8}
     & Fine-tuning 
    % & Fine-tune 
    & \textbf{\ours}-\textcolor{dark_blue}{70B} 
    & \textbf{56.75} & \textbf{49.90} &37.76 &\textbf{48.14} &\textbf{78.36} \\
    %  & Fine-tuning 
    % % & Fine-tune 
    % & {\ours}-\textcolor{dark_blue}{70B} (distilled)
    %  &  &  &  &  \\
\bottomrule
\hline
\end{tabular}}
\caption{\textbf{Overall performance of {\ours} on HotpotQA and ALFWorld.} The evaluation metrics are F1 Score (\%) and Success Rate (\%), respectively. \textbf{Strategy} means the agent learning paradigm behind each method. The best results of each backbone are marked in \textbf{bold}.
}
\label{tab:main_results1}
\end{table*}

